Not Now, Ask Later: Users Weaken Their Behavior Change Regimen Over Time, But Expect To Re-Strengthen It Imminently

How effectively do we adhere to nudges and interventions that help us control our online browsing habits? If we have a temporary lapse and disable the behavior change system, do we later resume our adherence, or has the dam broken? In this paper, we investigate these questions through log analyses of 8,000+ users on HabitLab, a behavior change platform that helps users reduce their time online. We find that, while users typically begin with high-challenge interventions, over time they allow themselves to slip into easier and easier interventions. Despite this, many still expect to return to the harder interventions imminently: they repeatedly choose to be asked to change difficulty again on the next visit, declining to have the system save their preference for easy interventions.

==> study3.tex <==
\section{Study 4: Effects of User Control}

Our previous experiments have focused on being able to accurately model user difficulty preferences, while attempting to minimize adverse effects from difficulty choice prompts. However, the implicit assumption we have made is that it is fundamentally desirable for behavior change systems to give users choices and follow them. That is, we have assumed that if a system can model and predict users' difficulty preferences, it should always give users interventions that match their preferences.

That said, there are reasons to suspect that blindly following user choices may often be suboptimal from a behavior change perspective. Users are present-biased in their choices, and will often make short-term choices that are not in line with their long-term goals~\cite{loewenstein1992choice, shu2010procrastination, ainslie2001breakdown, loewenstein1992choice, soman2005psychology}. Our results from our first study, where we observed that users' intervention selections decline in difficulty over time, are perhaps a reflection of this short-term decision making. The solution may be analogous to a personal fitness coach -- a coach may push us to go beyond what we think we can do or want in the moment; with the agreement on our part to cede some of our autonomy to the coach, we actually pay people to disrespect our in-the-moment wishes. Hence, reducing short-term user choices may potentially be beneficial for helping users achieve their long-term goals.

\subsection{Methodology}

In this experiment we study the effects of removing user choices, compared to providing them with choices. We do so by randomly assigning users to one of the following six conditions, two of which provide users with some level of choice as to the level of difficulty of their interventions, and four of which randomly assign users to be shown interventions of some difficulty level: % \msb{write out numbers under 100 unless it's in a data report} \geza{done}

\begin{itemize}
  \setlength\itemsep{0em}
    \item Non-choice conditions where users are randomly assigned a difficulty level for interventions:
\begin{itemize}
  \setlength\itemsep{0em}
    \item No interventions
    \item Easy interventions
    \item Medium interventions
    \item Hard interventions
\end{itemize}
\item Choice conditions:
\begin{itemize}
  \setlength\itemsep{0em}
  \item Initial choice: User initially chooses difficulty but does not subsequently update it
  \item Continuous choice: User chooses a difficulty initially and can subsequently update it via difficulty choice prompts, with the choice of when to ask again
\end{itemize}
\end{itemize}

We then compare these conditions based on retention as well as efficacy. We compare retention rates based on a Cox Hazard Regression model~\cite{cox1972regression}, and use a Linear Mixed Model (LMM)~\cite{nelder1972generalized} modeling time spent per day on the Facebook, where the user is a random effect, and condition is a fixed effect, as a means of comparing efficacy between the conditions. We chose to analyse results for Facebook because it is the site that is most commonly chosen as a goal, and we have the most interventions for it. For our intervention efficacy analysis, we only considered days where the user saw at least one intervention. % \msb{expand LMM for a nontechnical reader, since this is the first time you bring it up} \geza{done} \msb{this reads like it's a lmm with time \~{} (1|user). presumably you also at least need condition in there. any other variables in the model?} \geza{results <- lmer(logtime ~ condition + (1|user) + (1|domain), data = df)}

This study was conducted with 743 users, of whom 413 had Facebook as a goal site, over the course of 59 days. The mean install lifetime of a user was 17.2 days, median is 12 days, max install lifetime is 59 days, and standard deviation is 16.8. %Summing over the install lifetimes of all users, there were a total of 12798 days of observations. \msb{how long did this study last? how many people?}

\subsection{Results}

The retention results are shown in Figure~\ref{fig:nochoice_retention}. We observe that there are no significant differences between the conditions in terms of retention rates. Hence, randomly assigning users to harder or easier interventions by default, does not increase attrition.\footnote{Figure~\ref{fig:nochoice_retention} shows results from all users in the experiment, but if we restrict to only users who had Facebook as a goal, the results are identical.} % \msb{(or easier)} \geza{done}

\begin{figure*}
\centering
	\includegraphics[width=1.0\textwidth]{figures/nochoice_retention.png}
	\caption{Time spent per visit in each of the conditions -- initial choice, continuous choice, vs random assignments to various difficulty levels.} % retention_utils.ipynb
\label{fig:nochoice_retention}
\end{figure*}

The efficacy results are shown in Table~\ref{tab:nochoice_efficacy}. We observe that the most effective condition -- that is, the condition where time online is reduced the most -- is asking users for their initial intervention difficulty preference and giving them that difficulty. We suspect that the reason this is the most effective is that users' initial difficulty choice is harder than what they would choose long-term, as we saw in Study 1 (Figure~\ref{fig:difficulty_onboarding_percents}). As for why it would be more effective than assigning hard interventions by default, given that HabitLab allows users to disable interventions, we suspect that users assigned to interventions harder than they would prefer would end up disabling interventions at higher rates.

% The efficacy results are shown in Table~\ref{tab:nochoice_efficacy}. We observe that time online is reduced in the conditions where interventions are shown, and that assigning users to more difficult interventions by default improves efficacy. This confirms our expectations that interventions reduce time online, and that more difficult interventions are more effective. \msb{wait, this is not what the table says. the table says only initial user choice is a significant predictor}

% We observe that the most effective condition is asking users for their initial intervention difficulty preference and giving them that difficulty. We suspect that the reason this is the most effective is that users' initial difficulty choice is harder than what they would choose long-term, as we saw in Study 1 (Figure~\ref{fig:difficulty_onboarding_percents}). As for why it would be more effective than assigning hard interventions by default, given that HabitLab allows users to disable interventions, we suspect that users assigned to interventions harder than they would prefer would end up disabling interventions at higher rates. % The second most effective condition is assigning them to hard interventions \msb{we can't prove this with our stats --- I'd remove this part}, which we attribute to the power of defaults~\cite{brown2004skeptical, gallery2004superannuation, johnson2012beyond} -- even though the interventions might be more difficult than the user desires, inertia may still keep users from disabling them. The continuous experience sampling condition is the third most effective \msb{also can't prove this, could be random chance} -- we believe it is effective for the same reason as the initial choice condition, in that it is in line with the user's stated preference so they are less inclined to disable the interventions, but it is less effective as the user's choice of intervention difficulty falls over time, as we observed in Figure~\ref{fig:difficulty_over_time}. %we do not observe any significant difference between the conditions. Given the large number of participants and observations -- N users over N days, giving us N observations -- we believe this result may be due to limitations in the between-subjects approach to testing for efficacy. \geza{need to substitute visualization with the LMM}. \msb{right. it looks like actually doing nothing performs best?} \geza{actually now initial user choice performs best. but no significant differences.}

% \begin{figure}
% \centering
% 	\includegraphics[width=0.5\textwidth]{figures/nochoice_efficacy.png}
% 	\caption{Time spent per visit in each of the conditions -- initial user choice, continuous experience sampling, vs random assignments to various different difficulty levels. \geza{replaced with Table 1 -- as this result is averages}} % efficacy_utils.ipynb
% \label{fig:nochoice_efficacy}
% \end{figure}


% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: 四, 9月 19, 2019 - 02时53分51秒
% \begin{table}[!htbp] \centering 
% \begin{tabular}{@{\extracolsep{5pt}}lc} 
% \\[-1.8ex]\hline 
% \hline \\[-1.8ex] 
%  & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
% \cline{2-2} 
% \\[-1.8ex] & Log daily time on domain \\ 
% \hline \\[-1.8ex] 
%  Easy & 0.010 \\ 
%   & (0.058) \\ 
%   & \\ 
%  Medium & $-$0.057 \\ 
%   & (0.060) \\ 
%   & \\ 
%  Hard & 0.001 \\ 
%   & (0.058) \\ 
%   & \\ 
%  Continuous Exp. Sampling & $-$0.024 \\ 
%   & (0.057) \\ 
%   & \\ 
%  Initial User Choice & $-$0.068 \\ 
%   & (0.058) \\ 
%   & \\ 
%  Constant & 3.514$^{***}$ \\ 
%   & (0.045) \\ 
%   & \\ 
% \hline \\[-1.8ex] 
% Observations & 233,887 \\ 
% Log Likelihood & $-$447,590.400 \\ 
% Akaike Inf. Crit. & 895,198.700 \\ 
% Bayesian Inf. Crit. & 895,292.000 \\ 
% \hline 
% \hline \\[-1.8ex] 
% \textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
% \end{tabular} 
% 	\caption{Time spent per day on goal domains in each of the conditions -- initial user choice, continuous experience sampling, vs random assignments to various different difficulty levels. Baseline condition is where no intervention is shown.} % efficacy_utils.ipynb
%   \label{tab:nochoice_efficacy}
% \end{table} 

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: 四, 9月 19, 2019 - 12时35分39秒
%\begin{table}[!htbp] \centering 
\begin{table}[tb] \centering 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & Log daily time on Facebook \\ 
\hline \\[-1.8ex] 
 Assigned to Easy & $-$0.182 \\ 
  & (0.302) \\ 
  & \\ 
 Assigned to Medium & $-$0.223 \\ 
  & (0.310) \\ 
  & \\ 
 Assigned to Hard & $-$0.538 \\ 
% Assigned to Hard & $-$0.538$^{\dagger}$ \\ 
  & (0.307) \\ 
  & \\ 
 Initial User Choice & $-$0.615$^{*}$ \\ 
  & (0.298) \\ 
  & \\ 
 Continuous User Choice & $-$0.495 \\ 
% Continuous User Choice & $-$0.495$^{\dagger}$ \\ 
  & (0.298) \\ 
  & \\ 
 Constant & 5.323$^{***}$ \\ 
  & (0.228) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 3,524 \\ 
Log Likelihood & $-$6,688.215 \\ 
Akaike Inf. Crit. & 13,392.430 \\ 
Bayesian Inf. Crit. & 13,441.770 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.05; $^{**}$p$<$0.01; $^{***}$p$<$0.001} \\ 
% \textit{Note:}  & \multicolumn{1}{r}{$^{\dagger}$p$<$0.1; $^{*}$p$<$0.05; $^{***}$p$<$0.001} \\ 
\end{tabular} 
 	\caption{Daily time spent on Facebook in each of the conditions -- initial user choice, continuous difficulty choice prompts, vs random assignments to various different difficulty levels. The baseline condition is where no intervention is shown. Units are log-normalized seconds.} % \msb{Almost --- stargazer lets you set your p values that it reports. Get rid of 0.1 entirely --- it's not the norm in HCI to report alpha=.1, and will appear like you're trying to fool reviewers} efficacy_utils.ipynb % \msb{I hate that stargazer defaults to a * for p=.10. Change it to *=.05, **=.01, ***=.001} \msb{This might be clearer if you add some detail to Easy/Medium/Hard, e.g., ``Assigned to Easy''} \msb{doesn't this say the opposite of the abstract, which claims that randomizing to hard does best? here it says that just sticking with the initial pick is best --- presumably because of the initial over-optimism keeps things a little hard!}
   \label{tab:nochoice_efficacy}
\end{table} 
